GigaSpeechBench: A Real-World Multilingual Speech-to-Text Benchmark

While modern ASR systems achieve low error rates on high-resource benchmarks, such performance often overestimates real-world robustness. Existing evaluations address challenges in isolation, lacking a unified benchmark for domain terminology, age variation, dialects, accents, and low-resource languages, particularly across the Middle East and Southeast Asia, representing over one billion under-evaluated speakers. To address this gap, we introduce GigaSpeechBench, a comprehensive multilingual and multidimensional in-the-wild ASR & AST benchmark comprising 690 hours of human-annotated speech. It features five modules: (1) 12 low-resource Middle Eastern and Southeast Asian languages, plus challenging Japanese and Korean; (2) 6 Chinese dialects; (3) 6 English accents; (4) dense terminology across 12 vertical domains for Chinese and English; and (5) older adult and child speech. We further provide human-annotated Chinese and English translations for 11 languages to support AST evaluation. Extensive evaluations of leading foundation models and commercial APIs reveal significant performance degradation in these challenging settings, exposing critical evaluation blind spots.

==> table/Translate-AVG.tex <==
\begin{table}[t]
\centering
\caption{Average translation benchmark results across all evaluated countries. Each score is reported as English / Chinese. sacreBLEU, chrF++, COMET, and BLEURT are reported, where higher scores indicate better performance.}
\label{tab:translation_avg_results}
\renewcommand\tabcolsep{6pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule[1pt]
Model & sacreBLEU & chrF++ & COMET & BLEURT \\
\midrule

azure\_trans 
& 18.55 / 20.18 
& 40.05 / 13.92 
& 0.66 / 0.67 
& 0.54 / 0.48 \\

gemini-3-flash-preview
& \textbf{27.73 / 32.07} 
& \textbf{49.82 / 21.19} 
& \textbf{0.73 / 0.75} 
& \textbf{0.61 / 0.59} \\

seamless\_m4t\_v2\_large 
& 15.20 / 9.24 
& 34.18 / 7.21 
& 0.63 / 0.57 
& 0.51 / 0.33 \\

\bottomrule
\end{tabular}
}
\end{table}

==> table/duration.tex <==
\begin{table}[!t]
\centering
\small
\caption{Distribution of segment duration.}
\label{tab:duration_distribution}
% \renewcommand{\arraystretch}{1.1}
\begin{tabular}{lc}
\toprule[1pt]
Duration (s) & Ratio (\%) \\
\midrule
0.0--2.7   & 35.66 \\
2.7--5.4   & 22.47 \\
5.4--8.2   & 19.75 \\
8.2--10.9  & 15.25 \\
10.9--13.6 & 5.27  \\
13.6--16.3 & 1.58  \\
16.3+      & 0.01  \\
\bottomrule[1pt]
\end{tabular}
\end{table}

==> table/text_length.tex <==
\begin{table}[!t]
\centering
\small
\caption{Distribution of text length.}
\label{tab:text_length_distribution}
% \renewcommand{\arraystretch}{1.1}
\begin{tabular}{lc}
\toprule[1pt]
Length Interval & Ratio (\%) \\
\midrule
1--5   & 19.9 \\
5--20  & 43.6 \\
20--60 & 30.4 \\
60+    & 6.0  \\
\bottomrule[1pt]
\end{tabular}
\end{table}
